Evaluations of The Hierarchical Subspace Iteration Method

This document contains additional experiments concerned with the evaluation of the Hierarchical Subspace Iteration Method, which is introduced in~\cite{Nasikun2021}}

==> tables/detailed-model.tex <==
\begin{table}[t]
\begin{tabular}{|l|r|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Eigs}} & \multicolumn{4}{c|}{HSIM}                                                                                          \\ \cline{3-6} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{Hier.} & \multicolumn{1}{c|}{Solve} & \multicolumn{1}{c|}{\#Iter} & \multicolumn{1}{c|}{Total} \\ \hline \hline
\multirow{3}{*}{\shortstack[l]{Vase-Lion \\(200k)}}            & 50                                           & 3.2                       & 5.3                       & F|1                         & 8.5                       \\ \cline{2-6} 
                                             & 250                                          & 7.3                       & 41.2                      & F|2|1                       & 48.5                      \\ \cline{2-6} 
                                             & 1000                                         & 9.2                       & 188.0                     & F|3|1                       & 197.2                     \\ \hline
\multirow{3}{*}{\shortstack[l]{Knot-Stars\\(450k)}}           & 50                                           & 9.9                       & 28.4                      & F|1                         & 38.3                      \\ \cline{2-6} 
                                             & 250                                          & 29.1                      & 131.0                     & F|2|1                       & 160.1                     \\ \cline{2-6} 
                                             & 1000                                         & 36.3                      & 505.7                     & F|3|1                       & 542.0                     \\ \hline
\multirow{3}{*}{\shortstack[l]{Red-Circular\\(700k)}}         & 50                                           & 10.2                      & 65.5                      & F|1                         & 75.7                      \\ \cline{2-6} 
                                             & 250                                          & 40.6                      & 199.3                     & F|2|1                       & 239.9                     \\ \cline{2-6} 
                                             & 1000                                         & 36.3                          & 505.7                          & F|3|1                           & 542.0                          \\ \hline
\end{tabular}
\caption{The number of iterations for models with high details are in par with those models of smooth surface.}
	\label{tab:detail}
\end{table}
